How Does Supernet Help in Neural Architecture Search?

Weight sharing, as an approach to speed up architecture performance estimation has received wide attention. Instead of training each architecture separately, weight sharing builds a supernet that assembles all the architectures as its submodels. However, there has been debate over whether the NAS process actually benefits from weight sharing, due to the gap between supernet optimization and the objective of NAS. To further understand the effect of weight sharing on NAS, we conduct a comprehensive analysis on five search spaces, including NAS-Bench-101, NAS-Bench-201, DARTS-CIFAR10, DARTS-PTB, and ProxylessNAS. We find that weight sharing works well on some search spaces but fails on others. Taking a step forward, we further identified biases accounting for such phenomenon and the capacity of weight sharing. Our work is expected to inspire future NAS researchers to better leverage the power of weight sharing.

==> tables/correlation1.tex <==
\begin{tabular}{ccccccc}
  \toprule
        Budgets &  NB-101 &  NB-101-6M &  NB-201 &  NB-201-0.4M &  DARTS &  PTB \\
  \midrule
      1$\times$ &  0.4679 &     0.1989 & -0.1648 &      -0.0964 & 0.3660 &  NaN \\
      2$\times$ &  0.5077 &     0.2065 &  0.0167 &       0.0826 & 0.5404 &  NaN \\
      4$\times$ &  0.5458 &     0.2696 &  0.3430 &       0.3182 & 0.1729 &  NaN \\
      8$\times$ &  0.6185 &     0.3497 &  0.6408 &       0.5110 & 0.1204 &  NaN \\
     16$\times$ &  0.6587 &     0.4530 &  0.7143 &       0.5768 & 0.2038 &  NaN \\
     32$\times$ &  0.6164 &     0.3949 &  0.6716 &       0.5361 & 0.2047 &  NaN \\
     64$\times$ &  0.6070 &     0.3530 &  0.6771 &       0.5480 & 0.2208 &  NaN \\
    128$\times$ &  0.5952 &     0.3439 &  0.7006 &       0.5629 & 0.2476 &  NaN \\
    256$\times$ &     NaN &        NaN &  0.7193 &       0.5894 & 0.2396 &  NaN \\
  \midrule
     Parameters &  0.6727 &     0.5315 &  0.7489 &       0.4864 & 0.4113 &  NaN \\
   Ground Truth &  0.9852 &     0.9674 &  0.9945 &       0.9878 &    NaN &  NaN \\
  \bottomrule
\end{tabular}

==> tables/hparams-supernet.tex <==
\begin{tabular}{c|c|c|c|c|c}
    \hline
    & NB-101 & NB-201 & DARTS-C & Proxyless & DARTS-P \\
    \hline
    Batch size & 256 & 256 & 448$^*$ & 1024$^*$ & 256 \\
    Initial LR & 0.1 & 0.05 & 0.1 & 0.2 & 40 \\
    LR Decay   & Cosine & Cosine & Cosine & Cosine & Fixed \\
    Ending LR  & 0 & 0 & 0 & 0 & 40 \\
    Optimizer  & SGD & SGD & SGD & SGD & SGD/ASGD \\
    Momentum   & 0.9 & 0.9 & 0.9 & 0.9 & 0 \\
    Nesterov   & no  & yes & no  & no  & no \\
    Weight decay & 0.0001 & 0.0005 & 0.0003 & 0.0005 & $8 \cdot 10^7$ \\
    % Initial convolution filters & 128 & 16 & 36 & 40 & - \\
    Gradient clip & 5 & 5 & 5 & 0 & 0.1 \\
    Auxiliary weight & 0 & 0 & 0.4 & 0 & - \\
    Label smoothing~\cite{szegedy2016rethinking} & 0 & 0 & 0 & 0.1 & - \\
    Cutout~\cite{devries2017cutout}      & 0 & 0 & 16 & 0 & - \\
    Drop-Path Prob~\cite{larsson2016fractalnet}   & 0 & 0 & 0.2 & 0 & - \\
    BN calib batch size & 400 & 400 & 200 & 400 & - \\
    BN calib steps      & 25  & 25  & 100 & 25  & 0 \\
    \# GPUs       & 1 & 1 & 4 & 8 & 1 \\
    \hline
\end{tabular}

==> tables/performance1.tex <==
\begin{tabular}{c|c|cccc|cccc}
    \hline
    & & \multicolumn{4}{c|}{Supernet} & \multicolumn{4}{c}{Ground Truth} \\ \cline{3-10}
    Search Space &        Budgets &   Avg &  Best &  Worst & Range &   Avg &  Best &  Worst & Range \\
    \hline
    NB-101 &  148.1$\times$ & 91.21 & 94.22 &  64.51 & 29.71 & 90.71 & 94.53 &  34.38 & 60.16 \\
    NB-201 &   20.0$\times$ & 50.90 & 64.86 &  19.78 & 45.08 & 62.74 & 73.13 &   9.77 & 63.36 \\
     DARTS &   13.3$\times$ & 92.87 & 94.57 &  82.72 & 11.85 & 96.91 & 97.38 &  96.18 &  1.20 \\
 Proxyless &    3.3$\times$ & 73.26 & 74.90 &  67.74 &  7.15 & - &     - &      - &     - \\
       PTB &    1.3$\times$ & 66.31 &  64.75 & 71.57 & 6.81 & 60.04 & 57.87 &  63.88 &  6.01 \\
    \hline
\end{tabular}


==> tables/proxyless-structure.tex <==
% 1.3x

\begin{tabular}{c|c|c|c|c}
    \hline
    Input               & Block             & Expand Ratio  & Kernel Size   & Channels & Repeat & Stride \\
    \hline
    $224^2 \times 3$    & $3 \times 3$ Conv & -             & -             & 40       & 1      & 2 \\
    $112^2 \times 40$   & MBConv            & 1             & 3             & 24       & 1      & 1 \\
    \hline
\end{tabular}

==> tables/pruned1.tex <==
\begin{tabular}{c|c|cccc|cccc}
    \hline
    & & \multicolumn{4}{c|}{Ground Truth} & \multicolumn{4}{c}{Random} \\ \cline{3-10}
                 & Space &  Corr &  Perf &  Top1-Reg &  Top10-Reg &    Corr &  Perf &  Top1-Reg &  Top10-Reg \\
    \hline
     \multirow{5}{*}{NAS-Bench-101} &   9598 & 0.36 &  6.98 & 0.59 & 0.13 & 0.61 & 12.11 & 0.89 & 0.68 \\
     &  23996 & 0.40 &  7.12 & 0.75 & 0.57 & 0.59 & 11.68 & 0.74 & 0.22 \\
     &  47992 & 0.59 &  8.79 & 0.64 & 0.28 &  NaN &   NaN &  NaN &  NaN \\
     &  71988 & 0.52 &  9.48 & 0.72 & 0.48 & 0.59 & 11.70 & 0.56 & 0.56 \\
     &  86386 & 0.60 & 10.49 & 0.46 & 0.29 & 0.64 & 11.34 & 0.77 & 0.53 \\ \hline
      \multirow{5}{*}{NAS-Bench-201} &   1528 & 0.22 & 34.96 & 1.72 & 1.72 & 0.83 & 49.19 & 5.71 & 3.09 \\
      &   3821 & 0.28 & 38.88 & 4.15 & 2.21 & 0.69 & 52.24 & 3.29 & 3.29 \\
      &   7642 & 0.44 & 42.45 & 3.72 & 2.29 & 0.64 & 53.01 & 2.93 & 2.91 \\
      &  11463 & 0.58 & 48.65 & 4.73 & 3.87 & 0.65 & 53.84 & 4.53 & 3.40 \\
      &  13755 & 0.61 & 51.60 & 5.91 & 3.56 & 0.67 & 54.10 & 4.55 & 3.33 \\
    \hline
\end{tabular}


==> tables/supernetstab.tex <==
\begin{tabular}{c|c|c|c|c}
    \hline
                              Group & Corr-BL & Corr-GT $\uparrow$ ($\Delta$) & Top-10 $\uparrow$ ($\Delta$) & S-Perf $\uparrow$ ($\Delta$) \\
    \hline
    NAS-Bench-101 (1k epochs)       &   1.000 &                0.618 &                93.45 &                88.38 \\
    FairNAS~\cite{chu2019fairnas}   &   0.967 &  0.683 (\textcolor{blue}{+0.064}) &  93.64 (\textcolor{blue}{+0.19}) &   86.59 (\textcolor{red}{-1.79}) \\
    Multi-Path~\cite{pham2018efficient} &   0.963 &  0.626 (\textcolor{blue}{+0.007}) &  93.87 (\textcolor{blue}{+0.42}) &   85.99 (\textcolor{red}{-2.38}) \\
    LR=0.05, WD=$3 \cdot 10^4$      &   0.982 &   0.608 (\textcolor{red}{-0.010}) &   93.13 (\textcolor{red}{-0.32}) &  88.86 (\textcolor{blue}{+0.49}) \\
    Different Seed                  &   0.982 &  0.630 (\textcolor{blue}{+0.012}) &  93.59 (\textcolor{blue}{+0.14}) &   87.57 (\textcolor{red}{-0.80}) \\
    \hline
    NAS-Bench-101 (2k epochs)       &   1.000 &                0.659 &                93.82 &                90.58 \\
    FairNAS                         &   0.964 &   0.652 (\textcolor{red}{-0.007}) &   93.41 (\textcolor{red}{-0.41}) &   90.32 (\textcolor{red}{-0.26}) \\
    Multi-Path                      &   0.963 &   0.656 (\textcolor{red}{-0.002}) &   93.64 (\textcolor{red}{-0.18}) &   90.29 (\textcolor{red}{-0.29}) \\
    LR=0.05, WD=$3 \cdot 10^4$      &   0.970 &   0.611 (\textcolor{red}{-0.048}) &   93.45 (\textcolor{red}{-0.37}) &  90.58 (\textcolor{blue}{+0.01}) \\
    Different Seed                  &   0.979 &   0.644 (\textcolor{red}{-0.014}) &   93.45 (\textcolor{red}{-0.37}) &   90.29 (\textcolor{red}{-0.28}) \\
    \hline
    NAS-Bench-201 (2k epochs)       &   1.000 &                0.701 &                  69.66 &                  49.01 \\
    FairNAS &   0.978 &  0.716 (\textcolor{blue}{+0.015}) &  69.87 (\textcolor{blue}{+0.21}) &    48.74 (\textcolor{red}{-0.27}) \\
    Multi-Path &   0.984 &  0.706 (\textcolor{blue}{+0.005}) &  70.05 (\textcolor{blue}{+0.39}) &    48.73 (\textcolor{red}{-0.28}) \\
    CIFAR-10 &   0.915 &  0.831 (\textcolor{blue}{+0.130}) &  69.87 (\textcolor{blue}{+0.21}) &  81.95 (\textcolor{blue}{+32.94}) \\
    ImageNet-16-120 &   0.962 &  0.711 (\textcolor{blue}{+0.010}) &  69.72 (\textcolor{blue}{+0.06}) &   21.81 (\textcolor{red}{-27.20}) \\
    \hline
\end{tabular}


==> tables/top10-perf.tex <==
\begin{tabular}{c|ccc|ccc|cc|cc}
    \hline
    & \multicolumn{3}{c|}{NAS-Bench-101} & \multicolumn{3}{c|}{NAS-Bench-201} & \multicolumn{2}{c|}{DARTS} & \multicolumn{2}{c}{PTB} \\ \cline{2-11}
    \hline
           Epochs & Top-1 &  Top-10 &  Top-100 &  Top-1 &  Top-10 &  Top-100 &  Top-1 &  Top-10 &  Top-1 &  Top-10 \\
    \hline
               64 &       NaN &       NaN &       NaN &     30.15 &     29.74 &     28.39 &     2.93 &     2.52 &    NaN &    NaN \\
              128 &      7.14 &      7.14 &      5.80 &     32.71 &     30.63 &     28.68 &     2.96 &     2.61 &    NaN &  58.24 \\
              256 &      7.14 &      7.14 &      5.80 &     31.95 &     30.47 &     29.23 &     2.96 &     2.61 &  59.73 &  58.57 \\
              512 &      6.21 &      6.21 &      5.65 &     31.62 &     30.74 &     28.68 &     2.96 &     2.78 &  62.18 &  59.45 \\
               1k &      6.37 &      6.21 &      5.80 &     31.26 &     30.63 &     29.39 &     2.96 &     2.61 &  62.18 &  59.45 \\
               2k &      7.19 &      5.80 &      5.59 &     30.75 &     30.34 &     28.90 &     3.12 &     2.77 &  61.22 &  59.45 \\
               4k &      6.39 &      6.36 &      5.80 &     30.74 &     30.47 &     29.23 &     2.71 &     2.71 &  60.12 &  58.57 \\
    \hline
           Random &      9.29 &      6.40 &      5.81 &     37.26 &     30.10 &     28.34 &     3.09 &     2.76 &  60.04 &  58.53 \\
     Ground Truth &      5.84 &      5.47 &      5.47 &     26.87 &     26.87 &     26.87 &     2.62 &     2.62 &  58.02 &  58.02 \\
    \hline
\end{tabular}

==> tables/top10.tex <==
\begin{tabular}{c|cc|cc|cc|cc}
    \hline
     & \multicolumn{2}{c|}{NAS-Bench-101} & \multicolumn{2}{c|}{NAS-Bench-201} &
                        \multicolumn{2}{c|}{DARTS} & \multicolumn{2}{c}{PTB} \\ \cline{2-9}
    Budgets & 1\% &  10\% &  1\% &  10\% &  1\% &  10\% &  1\% &  10\% \\
    \hline
       1$\times$ &      84 &      12 &     144 &      23 &     40 &      5 &    NaN &    NaN \\
       2$\times$ &      34 &      14 &      41 &       5 &      9 &      7 &    NaN &    NaN \\
       4$\times$ &      39 &       1 &      51 &       1 &     45 &     28 &   90 &    4 \\
       8$\times$ &      11 &       1 &      82 &      23 &     37 &     13 &   73 &   15 \\
      16$\times$ &       5 &       5 &     125 &       9 &      7 &      7 &   62 &   11 \\
      32$\times$ &      81 &       1 &      44 &      13 &      8 &      2 &   66 &   10 \\
      64$\times$ &      66 &       1 &     113 &      23 &      8 &      5 &   64 &   11 \\
     128$\times$ &      21 &       1 &     110 &       2 &     12 &      7 &   66 &    5 \\
     256$\times$ &       NaN &       NaN &     122 &       7 &      8 &      4 &    NaN &    NaN \\
    \hline
          Random &      55.3 &       9.8 &      57.7 &      13.8 &     28.3 &      6.9 &   50.9 &   13.9 \\
    \hline
\end{tabular}

==> tables/worst-best-comparison.tex <==
\begin{tabular}{c|cc|cc|cc|cc}
    \hline
    {} & \multicolumn{2}{c|}{NAS-Bench-101} & \multicolumn{2}{c|}{NAS-Bench-201} & \multicolumn{2}{c|}{DARTS-CIFAR10} & \multicolumn{2}{c}{DARTS-PTB} \\ \cline{2-9}
    {} & 10\% & 30\% & 10\% & 30\% & 10\% & 30\% & 10\% & 30\% \\
    \hline
    Worst Prec & 0.54 & 0.70 & 0.06 & 0.71 & 0.3 & 0.47 & 0.3 & 0.20 \\
    Best Prec & 0.36 & 0.53 & 0.09 & 0.60 & 0.2 & 0.33 & 0.0 & 0.27 \\
    \hline
\end{tabular}


==> text/background.tex <==
\section{Preliminaries}
\label{sec:related-works}

\paragraph{Weight sharing based NAS.}

Weight sharing is essentially the technique to build a supernet that contains all the architectures in the search space as its submodels, in order to reduce the massive computational cost to train each architecture from scratch. To train the supernet, some works~\cite{brock2017smash,bender18understanding,guo2019single,chu2019fairnas,chu2019scarletnas,cai2019train} uniformly sample architectures in the supernet, the updated weights of each architecture are assigned back to the corresponding weights in supernet. Some works~\cite{pham2018efficient,cai2018proxylessnas,you2020greedynas} gradually adjust the sampling probability of the architectures to converge to a smaller set of architectures. Some other works~\cite{hu2020anglebased,liu2018darts,chen2019pdarts,xu2019pcdarts} build the supernet with architecture parameters, which reduces to a co-optimization problem of architecture parameters and supernet weights.

% Such sampling could be generated by an RL controller, like \cite{pham2018efficient,cai2018proxylessnas}, or a random strategy from a pruned search space~\cite{you2020greedynas,hu2020anglebased}. They can also be an attention-like~\cite{vaswani2017attention} combination of many submodels, as done in gradient-based methods~\cite{liu2018darts,chen2019pdarts,xu2019pcdarts}.

In our experiments, we adopt uniform sampling for training a supernet (i.e., single-path one shot), as it is a generalized approach and it can also be seen as a basic component of other advanced sampling methods. It helps understand the capacity of supernet training based on weight sharing by excluding other training tricks. In single-path one shot, an architecture is sampled per mini-batch with the objective of minimizing the expectation of loss, i.e.,

\begin{equation}
\label{eq:naive-single-path-opt-goal}
\E_{\alpha \sim \Arch} [ \Ls_{val} (\Net(\phi, \alpha)) ]
\end{equation}

where $\Arch$ is the architecture search space, $\phi$ is the supernet weights, and $\Net$ is the corresponding architecture using weights from supernet.

Generally speaking, after a supernet is trained, a search strategy takes over to sample architectures and evaluates their performance based on the weights from the supernet. By comparing the evaluation performance, the search strategy finally settles down to several architectures and retrains them from scratch independently to pick the best one~\cite{guo2019single,chu2019scarletnas,chu2019fairnas,chu2020mixpath,you2020greedynas,zhang2020deeper}, which is often referred to as ``retraining'' or ``architecture evaluation''. The underlying assumption is, what performs well on supernet also performs well after retraining. However, such correlation is still under debate and exactly the topic of this paper. More recent works~\cite{yu2020scaling,cai2019train} have claimed that their supernet can directly produce good-performing models without retraining. Though their proposals are ad hoc to specific search spaces, they can be classified into another category of weight sharing NAS due to the elimination of retraining phase.

\paragraph{Search space.}

To conduct a comprehensive analysis of weight sharing, we run single-path one shot supernet training on 5 search spaces, from small search spaces with tabular benchmarks to popular large-scale search spaces, spanning the domain of both computer vision and natural language processing. We show the a summary of all search spaces in \autoref{tab:search-space-summary}. More details will be explained in appendix, including the experiment setups we used for these search spaces respectively.

\begin{table}
    \caption{Summary of search spaces.}
    \label{tab:search-space-summary}
    \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{c|c|c|c|c}
        \hline
        & Valid space size & Dataset & Task & Space type \\
        \hline
        NAS-Bench-101 & 95985 & CIFAR-10 & Image classification & Cell-wise~\cite{zoph2018learning} \\
        NAS-Bench-201 & 15284 & CIFAR-100 & Image classification & Cell-wise \\
        DARTS-CIFAR10 & $2.76 \cdot 10^{20}$ & CIFAR-10 & Image classification & Cell-wise \\
        ProxylessNAS & $2.22 \cdot 10^{17}$ & ImageNet & Image classification & Chain-wise~\cite{zoph2016neural} \\
        DARTS-PTB & $2.64 \cdot 10^9$ & Penn Treebank & Language modelling & Cell-wise \\
        \hline
        % Valid space size & 95985 & 15284 & $2.76 \cdot 10^{20}$ & $2.22 \cdot 10^{17}$ & $2.64 \cdot 10^9$ \\ \hline
        % Dataset & CIFAR-10 & CIFAR-100 & CIFAR-10 & ImageNet & Penn Treebank \\ \hline
        % Task & \multicolumn{4}{c|}{Image classification} & Language modelling \\ \hline
        % Space type & \multicolumn{3}{c|}{Cell-wise~\cite{zoph2018learning}} & Chain-wise~\cite{} & Cell-wise \\
        % \hline
    \end{tabular}
    \end{adjustbox}
\end{table}

% \begin{enumerate}
%     \item {\bf NAS-Bench-101}: NAS-Bench-101~\cite{ying2019nasbench101} is a tabular benchmark designed for evaluation of NAS search strategies. Similar to NAS-Bench-1shot1 \cite{zela2020nasbench1shot1}, we pruned the NAS-Bench-101 to a sub-search-space with 95985 cells to make it compatible with weight sharing approaches. For the context of this paper, we simply refer to the pruned search space as NAS-Bench-101.
%     \item {\bf NAS-Bench-201}: NAS-Bench-201~\cite{dong2020nasbench201} is another tabular benchmark, designed to be compatible with one-shot NAS. NAS-Bench-201 is evaluated on 3 image classification datasets, for this paper, we use CIFAR100 only. The valid search space is 15284.
%     \item {\bf DARTS-CIFAR10}: On CIFAR10, DARTS~\cite{liu2018darts} used a similar architecture search space as NASNet~\cite{zoph2018learning} and ENAS~\cite{pham2018efficient}, which designed a normal cell and reduction cell. The whole search space has $2.76 \cdot 10^{20}$ candidates, largest of all five.
%     \item {\bf ProxylessNAS Space}: Invented by ProxylessNAS~\cite{cai2018proxylessnas}, the search space is built upon a MobileNetV2~\cite{sandler2018mobilenetv2} skeleton, and searches for kernel size in 3, 5 and 7, expand ratio in 3, 4 and 6 and to use skip-connect block, resulting in $6^5 \cdot 7^{16} = 2.22 \cdot 10^{17}$ candidate architectures. We use 1.35 as the default width multiplier to align with Proxyless-GPU baseline.
%     \item {\bf DARTS-PTB Cell}: On language modeling task, we use search space designed in \cite{liu2018darts, pham2018efficient} for sequence-to-sequence task of Penn Treebank (PTB). The search space constructs a RNN cell, with $8$ hidden states, containing $8! \cdot 4^8 = 2.64 \cdot 10^9$ candidate cells.
% \end{enumerate}

% More details will be explained in appendix, where we include the subtle differences of the search space we used and previous literature, and how we apply weight sharing on some tricky ones.

\paragraph{Metrics.}

We design the following metrics to assess the effectiveness of weight sharing in NAS:

\begin{itemize}[leftmargin=0.3in]
    \item {\bf Ground truth performance}: For architectures in search space, we train each one from scratch independently, obtaining performance on validation/test set, which we call \emph{ground truth performance}, \emph{ground truth} in short. We leverage existing tabular benchmarks for ground truths of NAS-Bench series, and train architectures on demand for others. %, which we will elaborate in appendix.
    \item {\bf Supernet performance}: To estimate a \emph{supernet performance} of an architecture, we first extract it from supernet, inheriting supernet weights, calibrate Batch-Norm statistics~\cite{guo2019single,bender18understanding,pourchot2020share,yu2020train}, and then evaluate it on the full validation set (top-1 accuracy for image classification task and perplexity for language modelling). If no architecture is specified, \emph{supernet performance} refers to the average performance of 1k architectures on supernet by default.
    \item {\bf Correlation}: Following \cite{yu2020train,pourchot2020share,zhang2020deeper,li2019random}, we show the correlation between supernet performance and ground truth performance. We will use Spearman correlation~\cite{spearman1961proof} in this paper. A higher correlation means better consistency. Correlations are calculated on a randomly sampled subset (1k for NAS-Bench series, 100 for DARTS series, 20 for ProxylessNAS).
    \item {\bf Top-$k$}: We randomly sample 1k architectures, choose top-$k$ based on supernet performance, and obtain their ground truth performance. We then use report test performance of the architecture with the best ground truth performance on validation set. % Note that such selection from a random subset can be easily replaced by other methods, such as evolutionary search and reinforcement learning~\cite{bender18understanding}.
\end{itemize}



==> text/body.tex <==
\section{Supernet: An Extensive Exploration}

\subsection{Performance and Correlation}

\autoref{eq:naive-single-path-opt-goal} suggests that to make weight sharing helpful in NAS, the supernet should be well optimized, or at least achieve a fair minimum. Previous works~\cite{chu2019fairnas,chu2019scarletnas,guo2019single,luo2019understanding} all use supernet performance as a quality indicator of architecture performance prediction. To verify the effectiveness of such practice, instead of using various tricks that claim to have boosted the supernet performance, we simply increase the training epochs (the effectiveness of longer training is also suggested by \cite{luo2019understanding}). Concretely, we repeatedly double the number of epochs, measuring supernet performance and correlation. As a result, we obtain a series of supernets as shown in \autoref{fig:correlation-error}.

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/correlation-error-nb201}
        \caption{NAS-Bench-201}
    \end{subfigure}
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/correlation-error-darts}
        \caption{DARTS-CIFAR10}
    \end{subfigure}
    \begin{subfigure}{0.39\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/correlation-error-nb101}
        \caption{NAS-Bench-101}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/correlation-error-proxyless}
        \caption{ProxylessNAS}
    \end{subfigure}
    \begin{subfigure}{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/correlation-error-ptb}
        \caption{DARTS-PTB}
    \end{subfigure}
    \caption{Supernet performance and correlations with respect to the number of epochs. The dotted line is the average ground truth performance, i.e., performance of architectures when they are trained independently. On ProxylessNAS, we could not get a fair number of ground truths, so correlations are not available, and we use the top-1 accuracy of Proxyless-GPU~\cite{cai2018proxylessnas} as the dotted line.}
    \label{fig:correlation-error}
\end{figure}

\paragraph{Supernet performance.} There is a clear trend that extended training can boost supernet performance on all five search spaces. On NAS-Bench-101, supernet performance even surpasses ground truth. On ProxylessNAS, the performance is only 2\% away from reference line at 1k epochs, and we expect such gap to be further narrowed if we had resources for more epochs. However, for other search spaces, such gap is still quite large, seemingly touching an upper bound. For example, on NAS-Bench-201, even if we train 4k epochs, which is 20$\times$ budget of a single model training, the gap is still as large as 10\%. On DARTS-CIFAR10, the improvement is more and more negligible as we further double the number of epochs. This result, together with the findings in \cite{yu2020scaling,cai2019train}, reveals that simultaneous optimization of tremendous architectures in one supernet is possible, yet it might require considerable computational cost and advanced optimization techniques.

\paragraph{Supernet correlation.} Despite the supernet performance on some search spaces looks better than others, the correlations are generally not high. Notably, on PTB, the correlation is lower than 0, meaning that the supernet even favors worse architectures. Although we observe an increase in correlation at the very beginning, it soon becomes saturated and further increasing the epochs can even harm the ranking quality. For example, on DARTS-CIFAR10, correlation achieves a 0.54 at 64 epochs, but later decreases to around 0.2 with further training. On PTB, the correlation is even worse as the supernet performance gets better. To summarize, there is a gap between the goal of supernet training (i.e., to minimize the expectation loss) and a better ranking model that distinguishes the good architectures from bad. A supernet that performs well for all architectures does not necessarily have the ability to rank the ground truth performance of architectures.

\paragraph{Supernet-suggested top.} However, it is still unclear whether a better-trained supernet can be more useful in NAS, because the overall ranking quality is only an intermediate metric. We then further examine the ground truth performance of the architecture selected based on the supernet, and show the results in \autoref{fig:top10-perf}. Though a better correlation usually yields a better top-1 and top-10, top performance is not sensitive to small changes in correlation. The top-1 architecture is almost constantly better than random architecture, while the advantage of top-10 seems weaker. Generally, supernet is indeed helpful to find a relatively good architecture, but usually struggles to find one of the best. Moreover, echoing the findings of correlation, extended training with more epochs hardly improves top-1 and top-10. Finally, comparing across search space, the effectiveness of weight sharing relies on the particular search space. DARTS-CIFAR10 seems the most friendly to supernet, whereas architectures found by DARTS-PTB are even worse than random.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{0.44\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/top1-top10-nb101}
        \caption{NAS-Bench-101}
    \end{subfigure}
    \begin{subfigure}{0.44\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/top1-top10-nb201}
        \caption{NAS-Bench-201}
    \end{subfigure}
    \begin{subfigure}{0.38\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/top1-top10-darts}
        \caption{DARTS-CIFAR10}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/top1-top10-proxyless}
        \caption{ProxylessNAS-600M}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/top1-top10-ptb}
        \caption{DARTS-PTB}
    \end{subfigure}
    \caption{We show the best ground truth over the top-1, and top-10 (top-5 for ProxylessNAS) architectures out of 1k recommended by the supernet. We also calculated a random search baseline, i.e., expectation of top-$k$ for a random rank. On NAS-Bench-101 and NAS-Bench-201, we further show the best ground truth out of 1k architectures. For DARTS-CIFAR10, PTB and ProxylessNAS, as the ground truths of all 1k architectures are unavailable, we skip this comparison. On ProxylessNAS, only architectures with FLOPs less than 600M are considered for this experiment.}
    \label{fig:top10-perf}
\end{figure}

\subsection{Bias of Weight Sharing}
\label{sec:bias}

In the previous section, we have shown that weight sharing can be, to some extent, useful in distinguishing good architectures from bad, but to what degree it is useful is closely related to the search space. For example, on NAS-Bench-101 and NAS-Bench-201, supernet works better than on DARTS-CIFAR10 and DARTS-PTB. In this section, we will further discuss what kind of architectures are favored by supernet.

We first verify the existence and consistency of such bias. In \autoref{fig:correlation-mutual}, we show mutual correlations between supernets and ground truths. Interestingly, some supernets enjoy a high mutual correlation despite the fact that they are trained with different epochs (e.g., 256, 1k and 4k epochs on NAS-Bench-201 and DARTS-CIFAR10) and training tricks (shown in appendix) --- they have a highly-agreeable rank on sampled architectures. It seems that architecture rank derived from supernet easily falls into a relatively stable state, where the rank stays almost unchanged as the optimization keeps going. However, this stable state can be nowhere near the rank of ground truth performance, forming the bias of weight sharing.

\paragraph{Bias towards big models.} It is well known that over-parameterized architectures, i.e., architectures with large number of parameters/FLOPs, usually enjoy a better ground truth performance~\cite{tan2019mnasnet,tan2019efficientnet}. As a result, for a search space containing small models and large models simultaneously (e.g., 1M to 13M parameters for NAS-Bench-101, 0.1M to 1.3M for NAS-Bench-201 and 2M to 4M for DARTS), model size can be a fairly good performance estimator baseline. As shown in \autoref{fig:correlation-mutual}, the correlation between ground truth performance and parameter size on NAS-Bench-101 can be as high as 0.67, outperforming all the attempts from supernet to estimate a good rank. Also, supernet performance has a higher correlation against parameter size than ground truth, which means supernet favors big models more than ground truth does. When we compare across all search spaces shown in \autoref{fig:correlation-mutual} (we will show more in appendix), we note that the correlations are generally higher when the parameter size is a good indicator of architecture performance. This implies that it is easier to reach a seemingly good correlation on an architecture space with variation in model size.

% For an ablation study, we limit the parameters on NAS-Bench-101 within 5.5M to 6.5M (\autoref{fig:correlation-mutual-nb101-6m}) to weaken the correlation between model size and performance. 

% there have been works addressing the issue that supernet favors large architectures~\cite{guo2019single,wu2019fbnet,cai2018proxylessnas}. As different search spaces have different parameter size variations (1M to 13M parameters for NAS-Bench-101, 0.1M to 1.3M for NAS-Bench-201, 2M to 4M for DARTS, and all same for PTB), for a search space with a large range of different scaled architectures, parameter size can actually be a fairly good ranking of ground truth performance. In \autoref{fig:correlation-mutual}, we look at the mutual correlations of ground truth, parameter size, and ranking reported by supernet trained with different epochs. We find that the correlation between ground truth performance and parameter size on NAS-Bench-101 can be as high as 0.75, outperforming all the attempts from supernet to predict a good rank. Such good correlation is weakened when we limit the parameters on NAS-Bench-101 within 5.5M to 6.5M (\autoref{fig:correlation-mutual-nb101-6m}). Moreover, comparing across all search spaces in \autoref{fig:correlation-mutual}, supernet can be better at ranking when the parameter size is a good indicator of architecture performance. We show more comparisons in appendix.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/correlation-mutual-nb101}
        \caption{NAS-Bench-101}
    \end{subfigure}
    % \begin{subfigure}{0.245\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/correlation-mutual-nb101-6m}
    %     \caption{NAS-Bench-101-6M}
    %     \label{fig:correlation-mutual-nb101-6m}
    % \end{subfigure}
    \begin{subfigure}{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/correlation-mutual-nb201}
        \caption{NAS-Bench-201}
    \end{subfigure}
    % \begin{subfigure}{0.325\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/correlation-mutual-nb201-04m}
    %     \caption{NAS-Bench-201-0.4M}
    %     \label{fig:correlation-mutual-nb201-04m}
    % \end{subfigure}
    \begin{subfigure}{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/correlation-mutual-darts}
        \caption{DARTS-CIFAR10}
    \end{subfigure}
    \begin{subfigure}{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/correlation-mutual-ptb}
        \caption{DARTS-PTB}
    \end{subfigure}
    \caption{Mutual correlation among supernet performances under different budgets (number of epochs), number of parameters (P) and ground truth performance (GT). As all architectures are of the same size for DARTS-PTB, parameters dimension is hidden.}
    \label{fig:correlation-mutual}
\end{figure}

\paragraph{Bias towards certain operators.} We note that supernet can bias towards some particular candidates that make itself easier to train but do not train well independently. We support this claim with the sampled architectures grouped by choice of certain operators, shown in \autoref{fig:bias}. For NAS-Bench-101, Conv3x3 is clearly preferred by supernet. Fortunately, architectures with Conv3x3 indeed have relatively good performance. On NAS-Bench-201 however, Conv3x3 is also greatly biased on the shortcut operator from input node to output node, but almost all architectures with best ground truth performance choose skip connection, which is why top-$k$ is low in \autoref{fig:top10-perf}. Similarly, on DARTS-PTB, Tanh, which is favored by supernet, turns out to be a worse option.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{0.325\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/bias-nb101}
        \caption{NAS-Bench-101 (Node 1)}
    \end{subfigure}
    \begin{subfigure}{0.325\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/bias-nb201}
        \caption{NAS-Bench-201 (Edge 0-3)}
    \end{subfigure}
    % \begin{subfigure}{0.325\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/bias-darts}
    %     \caption{DARTS-CIFAR10 (Left operator of 2nd node)}
    % \end{subfigure}
    \begin{subfigure}{0.325\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/bias-ptb}
        \caption{PTB (Activation of 2nd node)}
    \end{subfigure}
    \caption{Relationship between supernet performance and ground truth performance, grouped by decision on a specific operator, as stated in parenthesis. The most biased candidate is highlighted.}
    \label{fig:bias}
\end{figure}

\subsection{Pruned Search Space}

\paragraph{Effectiveness of Pruning.}

Intuitively, if a search space is smaller, there will be fewer distractions among architectures and supernet training will be more similar to stand-alone training. As weight sharing has the above-mentioned limitations from the aspects of supernet performance, correlation and bias on found architectures, we naturally seek to figure out whether such limitations still exist when a search space is gradually downscaled. To start with, we run experiments with different pruning ratios, using the following two approaches to prune NAS-Bench-101 and NAS-Bench-201 search space:

\begin{itemize}[leftmargin=0.3in]
    \item {\bf Optimistic Pruning}: Prune architectures with the worst ground truth performance.
    \item {\bf Random Pruning}: Prune a random part of search space.
\end{itemize}

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{0.38\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/pruned-best-nb101}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/pruned-best-nb101-corr}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/pruned-best-nb101-supernet}
    \end{subfigure}
    \begin{subfigure}{0.38\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/pruned-best-nb201}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/pruned-best-nb201-corr}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/pruned-best-nb201-supernet}
    \end{subfigure}
    \caption{We show experiments on NAS-Bench-101 in the first row and NAS-Bench-201 in the second row. We use blue for random pruning and black for optimistic pruning. Each point corresponds to an average of three trained supernets on one particular subspace and the error bars show the variance. The left two figures show top-10 found by supernet (solid line) and random search (dashed line). The blue dotted line corresponds to the best architectures in randomly-pruned search spaces. In the middle two figures, we show correlation with respect to ground truths. In the right two figures, we show average supernet performance and performance of the best architecture when directly evaluated on supernet. Pruning factor means by how many times the search space is downscaled.}
    \label{fig:prune-best}
\end{figure}

As observed from the optimistic cases (black lines) in \autoref{fig:prune-best} left, results are significantly better --- top-10 achieves better accuracy. However, in random cases (blue lines), meager improvement is observed. Combined with the fact that supernet correlation drops when the worst architectures in search space is pruned (\autoref{fig:prune-best} middle), we conjecture that, as the ground truth performance of remaining architectures are getting closer to each other, it will be harder to rank them correctly, and the improvement in top-10 can be mainly ascribed to better quality of search space, i.e., higher average ground truth performance. Such hypothesis is supported by the fact that supernet-top-10 (solid lines in \autoref{fig:prune-best} left) is closely related with random-top-10 (dashed lines), and supernet-guided search improves at the same pace as the improvement in random search.

Similar phenomenon is observed on DARTS-CIFAR10 search space. Since we do not have ground truth performance of all architectures and the search space is too large to enumerate, we use the searched architecture DARTS (second order)~\cite{liu2018darts} as a gold architecture, creating multiple differently-scaled pruned search spaces around it by fixing some of its choice blocks. We trained 2k epochs for each supernet (including the all-pruned single net). We estimate the search space quality by taking the mean of ground truth performance of 10 randomly sampled architectures. We show the results in \autoref{fig:pruned-best-darts-gt-vs-top10} and \autoref{fig:pruned-best-darts-perf-line}. Combined with the findings on NAS-Bench series, we note that, a subspace with better average ground truth performance produces a better top-10 performance, while a poorly or randomly pruned search space hardly has such guarantee.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{0.325\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/prune-best-darts-gt-vs-top10}
        \caption{DARTS-CIFAR10 Top-10}
        \label{fig:pruned-best-darts-gt-vs-top10}
    \end{subfigure}
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/prune-best-darts-perf-line}
        \caption{DARTS-CIFAR10 Supernet Perf}
        \label{fig:pruned-best-darts-perf-line}
    \end{subfigure}
    \begin{subfigure}{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/prune-best-proxyless-perf-line}
        \caption{ProxylessNAS}
        \label{fig:pruned-best-proxyless-perf-line}
    \end{subfigure}
    \caption{Left: relationship between average ground truth performance and supernet top-10 performance. Point size corresponds to search space size in log scale. Middle: performance with respect to search space size when DARTS-CIFAR10 search space is pruned in a optimistic way. Right: performance of supernet when we prune ProxylessNAS search space optimistically.}
    \label{fig:prune-best-darts}
\end{figure}

From the supernet performance perspective, we also report the mean and top supernet performance when we evaluate architectures directly inheriting supernet weights without any retraining. We did a similar experiment on ProxylessNAS search space. As shown in \autoref{fig:prune-best} right, \autoref{fig:pruned-best-darts-perf-line} and \autoref{fig:pruned-best-proxyless-perf-line}, smaller search space has a clear tendency to be trained better than a larger one, provided that the pruning has been done correctly (instead of randomly). Interestingly, it does not have to be a single neural network to reach a best accuracy. The best on DARTS-CIFAR10 (97.57\%) is achieved when 343 architectures simultaneously trained (\autoref{fig:pruned-best-darts-perf-line}), while the best on ProxylessNAS (75.04\%) comes from a supernet with 7 architectures (\autoref{fig:pruned-best-proxyless-perf-line}). Moreover, little difference is observed between best performance and average performance (less than 0.1\%), which implies, if the subspace is small enough so that architectures are no longer distinguishable, we should resort to refining our training approach. For example, we can simply train all the architectures simultaneously in a supernet, like \cite{yu2020scaling,cai2019train} did.

\paragraph{Weight sharing guided pruning.}

We have already shown the potential of pruned search space, provided that the pruning is done properly. Yet, to effectively identify the worst architectures in a search space remains a big challenge. Fortunately, as pointed out by \cite{hu2020anglebased,you2020greedynas,chen2019pdarts,zhang2020deeper}, weight sharing can effectively identify the worst. Echoing those findings, we also observed a similar phenomenon on NAS-Bench series. On NAS-Bench-101 for example, the precision of supernet to identify the worst 30\% architectures is around 70\%, which means about 70\% of the marked-worst architectures are indeed the worst ones (the precision to locate best 30\% is only about 50\%). However, we found that such precision is lowered on DARTS-CIFAR10 and DARTS-PTB. On DARTS-PTB, the numbers (around 20\%) are even lower than random baseline (30\%). Seemingly, the effectiveness of pruning still relies on correlation, i.e., the high-quality of global rank. If the supernet is a poor ranking model, it will not help pruning either. In appendix we will provide more empirical findings on this.

% Also worthy of note, we find that the best (top 10\%) architectures rarely appear in the predicted worst, making the pruning effective yet safe. 

% Moreover, we compared precisions across different pruning ratios (pruning the worst 10\%, 30\%, or only keeping the best 10\%, 30\%). As shown in \autoref{tab:worst-best-comparison}. It is not a surprise that a milder pruning strategy (e.g., discarding the worst ones) ends up with a better precision. In appendix, we will demonstrate more results on pruned search spaces and precision-recall curves to substantiate such claim. Such phenomenon implies that pruning ratio should be carefully chosen, to balance efficiency and effectiveness.

% \begin{table}[htbp]
%     \centering
%     \caption{Comparison of supernet's precision in identifying the worst architectures versus identifying the best architectures. Concretely, we find the top-$k$\% and bottom-$k$\% of the architectures based on supernet performance, and check how much percent of them actually belong to top-$k$\% or bottom-$k$\%. Supernet trained with 1k epochs are used by default.}
%     \label{tab:worst-best-comparison}
%     \input{tables/worst-best-comparison}
% \end{table}



==> text/conclusion.tex <==
\section{Related Work}

Over the past few years, many works have been trying to uncover the flaws in weight sharing based NAS. Several works~\cite{yu2019evaluating,li2019random,yang2019nas,zhang2020deeper,adam2019understanding,singh2019study} evaluated popular weight sharing algorithms including ENAS and DARTS and found that all these methods meagerly outperforms random baseline, thus stating that weight sharing is hardly helpful in NAS. Some works even claim that most NAS methods are unreproducible~\cite{li2019random} and improving training approaches is much more promising than searching for a better architecture~\cite{yang2019nas}. On the contrary, Bender et al. \cite{bender18understanding} discovered a positive relationship between supernet predictions and real accuracy of architectures. The follow-up works~\cite{chu2019fairnas,chu2020mixpath,luo2019understanding,hu2020anglebased} also adopted ranking correlation analysis to support their proposed NAS methods, which shows a decent result. Moreover, several weight sharing based NAS~\cite{you2020greedynas,guo2019single,zhang2018search} compared their approach with random search baseline, claiming that their methods are significantly better than random, which seemingly contradicts the findings in those analytical papers. 

% The effectiveness of weight sharing has been questioned for a long time.

Comparing all these works, we noticed that most researchers are using their own implementation of weight sharing algorithms, on their own tailored search spaces, and evaluating their own metrics. Such differences make them hard to compare. Very recently, owing to the emergence of two benchmarks NAS-Bench-101~\cite{ying2019nasbench101} and NAS-Bench-201~\cite{dong2020nasbench201}, there have been more solid works built on those benchmarks. Zela et al.~\cite{zela2020nasbench1shot1} and Pourchot et al.~\cite{pourchot2020share} revealed how different variations of NAS-Bench-101 bias the supernets differently. Yu et al.~\cite{yu2020train} conducted a review over weight sharing related techniques (e.g., sampling policies), providing guidelines on how to train a supernet. These works elaborated on NAS-Bench experiments and are complementary to our work.

\section{Conclusion}

In this paper, we give a comprehensive view of weight sharing in neural architecture search. Through our experiments, we have shown that weight sharing, though effective on some search spaces, can be limited on others. Weight sharing imposes a bias towards certain architectures and hardly finds the top ones, yet it still can be leveraged to identify the worst architectures, which we believe is a promising lead for further work. We hope our findings can inspire future researchers to enhance the effectiveness of weight sharing and design better NAS algorithms.


\section*{Broader Impact}

This research is expected to inspire the NAS community and researchers. Hopefully, it will drive the auto-design of neural networks and push the state-of-the-art of downstream tasks, including image classification, object detection, semantic segmentation, text classification, language modelling, etc.

% \begin{ack}
% Use unnumbered first level headings for the acknowledgments. All acknowledgments
% go at the end of the paper before the list of references. Moreover, you are required to declare 
% funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work). 
% More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2020/PaperInformation/FundingDisclosure}.


% Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
% \end{ack}


==> text/intro.tex <==
\begin{abstract}
    With the success of Neural Architecture Search (NAS), weight sharing, as an approach to speed up architecture performance estimation has received wide attention. Instead of training each architecture separately, weight sharing builds a supernet that assembles all the architectures as its submodels. However, there has been debate over whether the NAS process actually benefits from weight sharing, due to the gap between supernet optimization and the objective of NAS. To further understand the effect of weight sharing on NAS, we conduct a comprehensive analysis on five search spaces, including NAS-Bench-101, NAS-Bench-201, DARTS-CIFAR10, DARTS-PTB, and ProxylessNAS. Moreover, we take a step forward to explore the pruning based NAS algorithms. Some of our key findings are summarized as: (i) A well-trained supernet is not necessarily a good architecture-ranking model. (ii) Supernet is good at finding relatively good (top-10\%) architectures but struggles to find the best ones (top-1\% or less). (iii) The effectiveness of supernet largely depends on the design of search space itself. (iv) Comparing to selecting the best architectures, supernet is more confident in pruning the worst ones. (v) It is easier to find better architectures from an effectively pruned search space with supernet training. We expect the observations and insights obtained in this work would inspire and help better NAS algorithm design.
\end{abstract}

\section{Introduction}

Despite the rapid development of deep learning, neural architectures still highly depend on hand-design which needs expert knowledge. To relieve such effort, the idea of automatically designing neural networks by exploring a tremendous architecture space has been proposed. In recent years, neural architecture search (NAS) has attracted wide attention and achieved state-of-the-art performance on various tasks including image classification~\cite{zoph2018learning,tan2019mnasnet,cai2018proxylessnas,tan2019efficientnet} and natural language modelling~\cite{pham2018efficient,zoph2016neural,liu2018darts}. However, early NAS methods rely on a computationally-intensive training and evaluation process of hundreds of candidate architectures. For example, methods based on reinforcement learning (RL)~\cite{zoph2016neural,zoph2018learning,tan2019mnasnet} often take thousands of GPU days to complete.

To accelerate the search process, another family of methods called weight sharing emerges. Weight sharing builds all candidate architectures into a supernet where each architecture corresponds to a submodel. Once the supernet has been trained, architectures can be directly evaluated by inheriting weights from the supernet, thus saving the huge cost to train each architecture from scratch. By enabling weight sharing in neural architecture search~\cite{pham2018efficient,liu2018darts,cai2018proxylessnas,bender18understanding}, the search process can be cut to a few hours on a single GPU. 
%e.g., RL-based weight sharing~\cite{pham2018efficient}, gradient-based methods~\cite{liu2018darts,cai2018proxylessnas}, and other methods that decouple the optimization of supernet from architecture search~\cite{bender18understanding,guo2019single,chu2019fairnas,chu2019scarletnas,cai2019train}.

Weight sharing is built on the hypothesis that an architecture’s performance estimated within a supernet indicates its real performance. However, the effectiveness of weight sharing has long been questioned since the hypothesis lacks theoretical guarantee. Many analytical papers have conducted empirical analysis on whether and how weight sharing helps in finding the best architecture from a search space~\cite{bender18understanding,luo2019understanding,yu2019evaluating,yang2019nas,zhang2020deeper,pourchot2020share,yu2020train}. Though interesting phenomenon and valuable insights are delivered, the understanding of weight sharing still only touches a tip of the iceberg. Since most works adopted their own evaluation metrics on their own search space, a comprehensive and fair comparison between different search space has never been covered. Sometimes different works even draw contradictory conclusions~\cite{bender18understanding,li2019random}. In response to such issues, we conduct a more comprehensive study spanning five different search spaces: NAS-Bench-101~\cite{ying2019nasbench101}, NAS-Bench-201~\cite{dong2020nasbench201}, DARTS-CIFAR10, DARTS-PTB~\cite{liu2018darts}, and ProxylessNAS~\cite{cai2018proxylessnas}. The study reveals that weight sharing does not always deliver the identical effects on different search spaces. For some spaces, NAS process can benefit from weight sharing to find a good-performing architecture, while for some others, weight sharing hardly works. One of the deeper reasons we identified is that weight sharing is biased towards certain operators, connections and model sizes.

Even for some search spaces where weight sharing can help find good-performing architectures, the search process still struggles to identify the best ones. Therefore, some works resort to reducing search space in order to improve the probability of finding the best. Specifically, some of them build a dedicated (RL) model to gradually converge to a much smaller space~\cite{pham2018efficient}, while some others use heuristic methods to prune the space~\cite{you2020greedynas,hu2020anglebased,chen2019pdarts,li2019improving}. To understand how search space pruning helps in NAS, we conduct extensive experiments to compare search spaces with different sizes. It is observed that it is harder for weight sharing to produce better rank of architectures on smaller spaces. However, even with a poor rank, a smaller space indeed helps to find a better architecture, as long as the search space is properly pruned (i.e., good-performing architectures are kept while bad-performing architectures are pruned). We further found that supernet itself has high potential in guiding the pruning of search space.

To conclude, our contributions can be summarized as follows:

\begin{itemize}[leftmargin=0.3in]
    \item To the best of our knowledge, we are the first to conduct comprehensive study on five different search spaces, spanning from convolutional neural networks to recurrent neural networks. The pairwise comparison between different spaces reveals more convincing insights, and also explains some contradictory conclusions drawn from previous papers.
    \item To the best of our knowledge, we are the first to systematically analyze search space pruning. Our findings reveal that space pruning has great potential to improve weight sharing based NAS. % the effectiveness of weight sharing in NAS.
    \item We released a NAS benchmark containing more than 500 architectures where the ground truth performance of each architecture is also reported, which we expect will facilitate NAS research.
\end{itemize}


==> text/review.tex <==
\metareview{This paper got quite divergent reviews. One accept and three reject. The reviewers like the comprehensive empirical studies provided in this paper. The investigated problem is also important. \textbf{This paper studies the characteristic of supernet on five different search spaces and the experiments are sufficient.} However, 3 reviewers share similar concerns that the results are all from empirical studies and the observations have overlap with prior works. New insights are lacking in this paper. AC reads the paper and shares similar concerns with the reviewers. Though the empirical studies are helpful, what is the new contribution (to methodology or theory) of this paper is unclear and does not meet the acceptance bar of NeurIPS. This paper may fit some other venues more on empirical studies.}

\review{They study the characteristic of supernet on five different search spaces and the experiments are sufficient. \textbf{They release a NAS benchmark containing more than 500 architectures} even though they didn’t upload the source code yet.}

\review{This paper did a great job to show many interesting findings that are novel to the literature. I find the results \textbf{in weight sharing bias sections particularly interesting}. Super-net favors architectures with larger FLOPS and some operators are very intuitive but not yet studied in this field. In general, I favor this line of research showing more concrete and detailed analysis, even only empirical, rather than building on top of a fragile foundation.}

\review{1. The performed experiments are comprehensive on the given several settings including different search spaces and datasets. The search spaces cover both convolutional neural networks and recurrent neural networks. The datasets involve CIFAR-10, CIFAR-100, ImageNet and Penn Treebank. \\ 2. Inspiring conclusions on supernet methods are obtained from the performed experiments and could be helpful for the future NAS development. The key findings can be summarized as: \textbf{1) a well-trained supernet does not necessarily hold a real rank of architectures. 2) the top architectures are easily found in the supernet but the best one is tough. 3) the effectiveness of the supernet largely depends on the search space design. 4) the pruning strategy is found useful in supernet-based NAS.} \\ 3. This paper systematically study the supernet-based NAS methods. Some conclusions are obtained from a series of experiments in the paper, which could be helpful for the future development of weight-sharing NAS. This paper leads researchers to comprehensively analyze the effect of the supernet method.}

